Assuring Safety of Vision-Based Swarm Formation Control

Vision-based formation control systems are attractive because they can use inexpensive sensors and can work in GPS-denied environments. The safety assurance for such systems is challenging: the vision component's accuracy depends on the environment in complicated ways, these errors propagate through the system and lead to incorrect control actions, and there exists no formal specification for end-to-end reasoning. We address this problem and propose a technique for safety assurance of vision-based formation control: First, we propose a scheme for constructing quantizers that are consistent with vision-based perception. Next, we show how the convergence analysis of a standard quantized consensus algorithm can be adapted for the constructed quantizers. We use the recently defined notion of perception contracts to create error bounds on the actual vision-based perception pipeline using sampled data from different ground truth states, environments, and weather conditions. Specifically, we use a quantizer in logarithmic polar coordinates, and we show that this quantizer is suitable for the constructed perception contracts for the vision-based position estimation, where the error worsens with respect to the absolute distance between agents. We build our formation control algorithm with this nonuniform quantizer, and we prove its convergence employing an existing result for quantized consensus.

==> appx-geometric-vision.tex <==
\subsection{Rigid-body transformation}
We use the rotation matrix $\RotM_i$ and the translation vector $\tvec_i$ to denote the transformation from the common North East Down world frame~(NED) to the camera frame of drone $i$.
Given a point with the coordinate $\FP = [x\, y\, z]^T$ in the world frame,
its coordinate $(\FP)_i$ in the camera frame of  $i$ is computed as:
\[
(\FP)_i = \RotM_i \FP + \tvec_i
\]
The relative transformation from the camera frame of drone $i$ to drone $j$ is then derived as
the rotation $\RotM_{ij} = \RotM_j\RotM_i^{-1}$
and the translation $\tvec_{ij} = \tvec_j - \RotM_{ij}\tvec_i$.
That is,
\[
(\FP)_j = \RotM_{ij} (\FP)_i + \tvec_{ij}
\]

Further, we denote the coordinate of the camera of drone $i$ \emph{in the world frame} as $\Og_i$.
By definition, we know $(\Og_i)_i = \mathbf{0}^T$ and $\Og_i = -\RotM_i^{-1}\tvec_i$.

\subsection{Geometric model for 3D vision}

We consider the ideal pinhole camera model (Chapter 3 in~\cite{ma2003invitation}) for the image forming process of each camera.
Given a point with the coordinates $\FP = [x\, y\, z]^T$ in the world frame,
Equation (3.18) in~\cite{ma2003invitation} gives the pixel coordinates using the camera intrinsic matrix $\CamM_i$ and rigid-body transformation.
We consider the rotation matrix $\RotM_i$ and the translation vector $\tvec_i$ from the world frame to the camera frame of drone $i$.
The coordinate $\pix_i = [u_i\, v_i\, 1]^T$ in the pixel coordinate frame~(PCF) of the drone $i$ are calculated with:
\[
s_i \pix_i
= [\CamM_i\; \mathbf{0}] \left[\begin{matrix} (\FP)_i \\ 1 \end{matrix}\right]
= [\CamM_i\RotM_i\; \CamM_i\tvec_i] \left[\begin{matrix} \FP \\ 1 \end{matrix}\right]
\]
where $s_i$ is the unknown depth of the point in PCF due to the projection from 3D to 2D.

\subsection{Relative displacement estimation for drone formation}

The true relative 2D displacement from drone $i$ to $j$ in the world frame, that is, \truij, can be inferred in the following way.
Without loss of generality, we assume the drone $i$ maintains the altitude $\alt_i$,
and the feature point \FP for relative pose estimation are on the ground, i.e., $\FP = [x\, y\, 0]^T$.
When we look out from the origin $\Og_i$,
the pixel $\pix_i$ and the feature point \FP must lie on the same ray disregarding the depth $s_i$.
That is, the following two unit vectors must be the same in the world frame:
\begin{equation}\label{eq:same-dir}
\frac{\overrightarrow{\Og_i\FP}}{\lVert\overrightarrow{\Og_i\FP}\rVert} = \RotM_i^{-1} \left(\frac{\CamM_i^{-1}\pix_i}{\lVert\CamM_i^{-1}\pix_i\rVert}\right)    
\end{equation}

\newcommand{\unitz}{\ensuremath{\hat{k}}\xspace}

Because we assume the drone maintains the altitude $\alt_i$ and \FP is on the ground,
if we have the relative angle $\theta_i$ between $\overrightarrow{\Og_i\FP}$ and Z-axis,
we can derive the length $\lVert\overrightarrow{\Og_i\FP}\rVert$ by
\[
\lVert\overrightarrow{\Og_i\FP}\rVert =  \frac{\alt_i}{\cos\theta_i}
\]
Further, because we know the unit vectors are the same from Equation~\eqref{eq:same-dir},
we can use the inner product with the unit vector $\unitz = [0\,0\,1]^T$ of Z-axis to obtain $\cos\theta_i$:
\[
\cos\theta_i
= \frac{\langle \unitz^T\RotM_i^{-1}, \CamM_i^{-1}\pix_i \rangle}{\lVert\unitz^T\RotM_i^{-1}\rVert\lVert\CamM_i^{-1}\pix_i\rVert}
= \frac{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i}{\lVert\CamM_i^{-1}\pix_i\rVert}
\]
where $\lVert\unitz^T\RotM_i^{-1}\rVert = 1$ because the length of \unitz is 1 regardless of the rotation $\RotM_i^{-1}$.

Therefore,
\begin{align}\label{eq:pix-to-fp}
\overrightarrow{\Og_i\FP} &= \lVert\overrightarrow{\Og_i\FP}\rVert \cdot \RotM_i^{-1} \left(\frac{\CamM_i^{-1}\pix_i}{\lVert\CamM_i^{-1}\pix_i\rVert}\right) \nonumber \\
                          &= \frac{\alt_i}{\cos \theta_i} \cdot \left(\frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\lVert\CamM_i^{-1}\pix_i\rVert}\right) \nonumber \\
                          &= \alt_i \cdot \left(\frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i}\right)
\end{align}

Finally, since $\RotM_j^{-1} = \RotM_i^{-1}\RotM_{ij}^{-1}$,
\begin{align}\label{eq:true-rel-pos}
\nonumber
\truij &= \overrightarrow{\Og_i\Og_j} = \overrightarrow{\Og_i\FP} + \overrightarrow{\FP\Og_j} = \overrightarrow{\Og_i\FP} - \overrightarrow{\Og_j\FP} \\ \nonumber
&= \alt_i \cdot \frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i}
 - \alt_j \cdot \frac{\RotM_j^{-1}\CamM_j^{-1}\pix_j}{\unitz^T \RotM_j^{-1}\CamM_j^{-1}\pix_j} \\
&= \alt_i \cdot \frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i}
 - \alt_j \cdot \frac{\RotM_i^{-1}\RotM_{ij}^{-1}\CamM_j^{-1}\pix_j}{\unitz^T \RotM_i^{-1}\RotM_{ij}^{-1}\CamM_j^{-1}\pix_j}
\end{align}
\chiao{TODO: projection to XY-plane}

The relative rotation $\RotM_{ij}$ can be estimated with any of relative pose estimation algorithms such as~\cite{nister2004relativepose} and \cite{li2006fivepoint}.

However, the ego drone $i$ may not have accurate $\CamM_j$ or $\alt_j$ of the other drone $j$.
The measurement of the orientation $\RotM_i$ and $\RotM_{ij}$ may also have noises.
Therefore, the estimation algorithms often use assumptions to simplify Equation~\eqref{eq:true-rel-pos}.
We will further discuss in Section~\ref{sec:perc-error} how perception error bound can be derived when assumptions are used.



In this section, we study the error bound on $\lVert \estij - \truij \rVert$
due to the following assumptions:
\begin{itemize}
    \item The ego drone $i$'s camera aligns with the NED world coordinate and points downward perfectly.
    \item All drones use the same camera intrinsic matrix $\CamM_i = \CamM_j = \CamM$.
    \item All drones maintains the same altitude $\alt_i = \alt_j = \alt$.
\end{itemize}

The orientation matrix $\RotM_i$ is the identity matrix.
The estimate \estij is obtained with a simplified version of Equation~\eqref{eq:true-rel-pos}:
\begin{equation}\label{eq:est-rel-pos}
\estij = \alt \cdot \frac{\CamM^{-1}\pix_i}{\unitz^T \CamM^{-1}\pix_i}
       - \alt \cdot \frac{\RotM_{ij}^{-1}\CamM^{-1}\pix_j}{\unitz^T \RotM_{ij}^{-1}\CamM^{-1}\pix_j}
\end{equation}
We aim to find the upper bound for perception error by searching for the worst pair of pixels $\pix_i$ and $\pix_j$ such that $\lVert \estij - \truij \rVert$ is maximized.

\begin{figure}
    \centering
    \chiao{TODO: illustration of feature points in common camera view.}
    \caption{Common camera view}
    \label{fig:common-view}
\end{figure}

First, we observe that the pair of pixels $\pix_i$ and $\pix_j$ must come from the same feature point \FP visible to both cameras on drone $i$ and $j$.
Therefore, we can confine the search space in the common view of the two cameras as shown in Figure~\ref{fig:common-view}. For a given pixel on the image plane, it's coordinate $\pix_i = [u_i, v_i, 1]^T$ in the pixel coordinate frame (PCF) should satisfy $0\leq u_i \leq W$ and $0\leq v_i \leq H$ where $W$ and $H$ are the width and height of the image. In addition, we can obtain the position of the corresponding feature point for the pixel as 
\begin{equation}
    P_i = \alt_i \cdot \frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i} - \RotM_i^{-1}\tvec_i
\end{equation}
Therefore, all feature points that can be viewed by the $ith$ camera is given by 
\begin{equation}
\begin{split}
    \mathbb{P}_i = &\{\\
                   & \hspace{2em} P_i \mid \\
                   & \hspace{2em} P_i = \alt_i \cdot \frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i} - \RotM_i^{-1}\tvec_i,\\ 
                   & \hspace{2em} \pix_i = [u_i, v_i, 1]^T,\\ 
                   & \hspace{2em} 0\leq u_i \leq W,\\ 
                   & \hspace{2em} 0\leq v_i \leq H\\ 
                   &\}
\end{split}
\end{equation}
Similarly, we can obtain the region that can be viewed by the $j$-th camera $\mathbb{P}_j$. Therefore, the common viewing region will be the intersection of $\mathbb{P}_i$ and $\mathbb{P}_j$. 

With the definition of the of the common viewing region from two cameras, we can define the optimization problem that maximize the perception error
\begin{equation}
\begin{split}
\min_{u_i, v_i, u_j, v_j} \quad & -\lVert \estij - \truij \rVert\\
\textrm{s.t.} \quad & \estij = \alt \cdot \frac{\CamM^{-1}\pix_i}{\unitz^T \CamM^{-1}\pix_i}
       - \alt \cdot \frac{\RotM_{ij}^{-1}\CamM^{-1}\pix_j}{\unitz^T \RotM_{ij}^{-1}\CamM^{-1}\pix_j}, \\
       & \pix_i = [u_i, v_i, 1]^T,\\
       & \pix_j = [u_j, v_j, 1]^T,\\
       & 0\leq u_i \leq W, \\
       & 0\leq v_i \leq H, \\
       & 0\leq u_j \leq W, \\
       & 0\leq v_j \leq H, \\
       & \alt_i \cdot \frac{\RotM_i^{-1}\CamM_i^{-1}\pix_i}{\unitz^T \RotM_i^{-1}\CamM_i^{-1}\pix_i} - \RotM_i^{-1}\tvec_i\\ 
       & = \alt_j \cdot \frac{\RotM_j^{-1}\CamM_j^{-1}\pix_j}{\unitz^T \RotM_j^{-1}\CamM_j^{-1}\pix_j} - \RotM_j^{-1}\tvec_j
\end{split}
\end{equation}
The optimization objective was to maximize the difference between estimated $\estij$ and actual $\truij$. The constraints for the optimization is given by the fact that the pixels should lie inside of both image planes and the pixels on both image planes map to the same feature point.


==> sec-experiment.tex <==
\section{Experiments}
\label{sec:experiment}
\newcommand{\ThreeDrones}{{three drones}\xspace}
\newcommand{\FourDrones}{four drones\xspace}

In our experiments, we aim to validate two claims:
\begin{inparaenum}[(1)]
\item The safe separation and formation are ensured by Theorem~\ref{thm:rel-pos-bound} and Proposition~\ref{prop:safety}.
\item The analysis of ultimate bounds is robust against varying \ApproxAbs{}s from different environments.
\end{inparaenum}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|c|c}
%                      & Initial Positions & Desired Formation \\ \hline
%         \ThreeDrones & [(0,-6),(0,0),(0,6)] & [(0,-2.5),(4.33,0),(0,2.5)]\\ \hline
%         \FourDrones  & [(0,-6),(0,-2),(0,2),(0,6)]& [(0,-2.5),(5,-2.5),(0,2.5),(5,2.5)] 
%     \end{tabular}
%     \caption{Initial positions and desired formation for three and four drones. }
%     \label{tab:exp-settings}
% \end{table}

\paragraph*{Experiment Setup}
We present the results from two experiment settings with three and  four drones.
For \ThreeDrones, the drones will be placed initially in a line with 6m interval between drones and form an equilateral triangle with edge length 5m. For \FourDrones, the drones are placed initially in a line with 4m interval and form a square with edge length 5m. Then, we simulate each formation for 10 runs in environment \AirSimNH under different environmental parameters by varying the fog level in the scenario. The \ApproxAbs{}s are obtained by random sample pairs of images in each of the environment.

We conduct our experiments on a workstation with Intel Core i7-10700K @ 3.80GHz, 32GB main memory, and Nvidia GTX1080Ti GPU installed with Ubuntu 20.04 LTS, Python 3.8, and OpenCV 4.6.0.
We use the Python API for the v1.8.1-Linux version of the \AirSim simulator~\cite{shah2018airsim}.


\subsection{Safety Assured Formation}
\label{subsec:experiment-bounded}

\begin{figure}[ht!]
    % \includegraphics[width=0.25\columnwidth, height=3.4cm]{figs/3drones-abs-pos.png}
    % \includegraphics[width=0.73\columnwidth, height=3.4cm]{figs/True_Relative_Distance.png}
    \centering
    \includegraphics[width=0.35\columnwidth, height=3.9cm]{figs/4drones-abs-pos.png}
    \includegraphics[width=0.63\columnwidth, height=3.9cm]{figs/4drones-rel-dist.png}
    \centering
    \caption{
    Absolute position~(\emph{Left}) from one simulation run and relative distance between pairs of drones for 10 simulation runs~(\emph{Right}) for four drones in environment \AirSimNH with no fog. For the plot on the left, each color represents the absolute position of a drone. For the plot on the right, each row shows true relative distance $\lVert\truij\rVert$ ({\color{blue}Blue} region), desired distance $\lVert\tgtij\rVert$ ({\color{green}Green} dashed lines), and derived ultimate bounds for safety and closeness using approximate abstractions ({\color{red}Red} lines).
     }
     \label{fig:rel-pos}
\end{figure}


We validate our claim that each pair of drones will maintain a relative distance $\lVert\truij\rVert$ around the distance $\lVert\tgtij\rVert$ specified for the formation. 
Figure~\ref{fig:rel-pos} shows results for \FourDrones formation. The trajectories of drones are on the left,
and true relative distances evolving with time for all six pairs of drones are on the right.
The trajectories show the drone still attempting to form the desired shapes under perception error.
On the right, we see that the true relative distance can get really close to the ultimate bound in several simulation runs.
Nevertheless, the system never leaves the ultimate bound,
and this is consistent with our analysis that entering the ultimate bound ensures formations and safe separation.


\subsection{Robustness of Ultimate Bound Analysis}
\label{subsec:experiment-envs}

\begin{figure}[ht!]
    \includegraphics[width=0.76\columnwidth]{figs/True_Relative_Distance_env_three_bounds.png}
    \centering
    \caption{
Relative distance between three pairs of drones for 10 simulation runs under three different levels of fog (level $0$ {\color{blue}Blue}, level $0.01$  {\color{green}Green}, and level $0.02$ {\color{red}Red}).
The upper and lower bound on distances is not violated with the change of environmental parameters. 
    }\label{fig:weather-condition}
\end{figure}

In this section, we look at how robust is our analysis across environmental variations. We vary the weather condition by adding different amounts of fog. We experiment with three different fog levels, 0, 0.01, and 0.02, and derive the \ApproxAbs{} from sampled data under each weather condition.  
We obtain the ultimate bound and repeat the same simulation.
The simulated result is shown in Figure~\ref{fig:weather-condition}.
We observe that even with the fog introduced,
the true relative distance between each pair of drones will still not exceed the ultimate bound derived for the corresponding environment.
We also observe that in a foggier environment, where the performance of the vision component worsens,
the formation becomes less stable.
In the meantime, the ultimate bound becomes more conservative,
preventing the relative distance from violating the bound.
Note that when the bound becomes larger than the desired relative distance between drones,
the lower bound on distances can go below 0.
In this case, the premise of Proposition~\ref{prop:safety} is no longer satisfied,
and the drones may actually collide.

